Fast Video Classification via Adaptive Cascading of Deep Models

Recent advances have enabled "oracle" classifiers that can classify across many classes and input distributions with high accuracy without retraining. However, these classifiers are relatively heavyweight, so that applying them to classify video is costly. We show that day-to-day video exhibits highly skewed class distributions over the short term, and that these distributions can be classified by much simpler models. We formulate the problem of detecting the short-term skews online and exploiting models based on it as a new sequential decision making problem dubbed the Online Bandit Problem, and present a new algorithm to solve it. When applied to recognizing faces in TV shows and movies, we realize end-to-end classification speedups of 2.4-7.8x/2.6-11.2x (on GPU/CPU) relative to a state-of-the-art convolutional neural network, at competitive accuracy.

==> cvpr/ack.tex <==
\section{Acknowledgment}
\label{s:ack}


==> cvpr/cmds.tex <==
\renewcommand{\ttdefault}{pxtt}

\newcommand{\URL}{\url}
\newcommand{\cc}[1]{\mbox{\smaller[0.5]\texttt{#1}}}

%\clubpenalty=10000
%\widowpenalty=10000

%\linespread{1.2}

\fvset{fontsize=\scriptsize,xleftmargin=8pt,numbers=left,numbersep=5pt}

\input{code/fmt}
\newcommand{\figrule}{\hrule width \hsize height .33pt}
\newcommand{\coderule}{\vspace{-0.4em}\figrule}

\setlength{\abovedisplayskip}{0pt}
\setlength{\abovedisplayshortskip}{0pt}
\setlength{\belowdisplayskip}{0pt}
\setlength{\belowdisplayshortskip}{0pt}
\setlength{\jot}{0pt}

\def\Snospace~{\S{}}
\renewcommand*\sectionautorefname{\Snospace}
\def\sectionautorefname{\Snospace}
\def\subsectionautorefname{\Snospace}
\def\subsubsectionautorefname{\Snospace}
\def\chapterautorefname{\Snospace}
%\renewcommand{\figurename}{Fig.}
%\def\figureautorefname{\figurename}
\newcommand{\subfigureautorefname}{\figureautorefname}

%\numberwithin{equation}{section}
\newcommand{\yes}{Y}
\newcommand{\no}{}

% sema
\newcommand{\shl}{\ \cc{<}\cc{<}\ }
\newcommand{\shr}{\ \cc{>}\cc{>}\ }

\if 0
\renewcommand{\topfraction}{0.9}
\renewcommand{\dbltopfraction}{0.9}
\renewcommand{\bottomfraction}{0.8}
\renewcommand{\textfraction}{0.05}
\renewcommand{\floatpagefraction}{0.9}
\renewcommand{\dblfloatpagefraction}{0.9}
\setcounter{topnumber}{10}
\setcounter{bottomnumber}{10}
\setcounter{totalnumber}{10}
\setcounter{dbltopnumber}{10}
\fi

\newif\ifdraft\drafttrue
\newif\ifnotes\notestrue
\ifdraft\else\notesfalse\fi

% ref. http://en.wikibooks.org/wiki/LaTeX/Colors
\newcommand{\TK}[1]{\textcolor{LimeGreen}{TK: #1}}
\newcommand{\XXX}[1]{\textcolor{red}{XXX: #1}}
\newcommand{\TODO}[1]{\textcolor{Melon}{TODO: #1}}

% hide comments
% \renewcommand{\TK}[1]{\ignorespaces}
% \renewcommand{\XXX}[1]{\ignorespaces}
% \renewcommand{\TODO}[1]{\ignorespaces}

%% Ensure ligatures (e.g., ``fine official flag'') can be copy/pasted from PDF.
\input{glyphtounicode}
\pdfgentounicode=1

\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}p{#1}}

% include macros
\newcommand{\includepdf}[1]{
  \includegraphics[width=\columnwidth]{#1}
}
\newcommand{\includeplot}[1]{
  \resizebox{\columnwidth}{!}{\input{#1}}
}

% list
\newcommand{\squishlist}{
\begin{itemize}[noitemsep,nolistsep]
  \setlength{\itemsep}{-0pt}
}
\newcommand{\squishend}{
  \end{itemize}
}

%%
%% NOTE.
%%  to use circled number in caption, use
%%   (e.g., \protect\C{1})
%%
\usepackage{tikz}
\newcommand*\C[1]{%
\begin{tikzpicture}[baseline=(C.base)]
\node[draw,circle,inner sep=0.2pt](C) {#1};
\end{tikzpicture}}

\newcommand*\BC[1]{%
\begin{tikzpicture}[baseline=(C.base)]
\node[draw,circle,fill=black,inner sep=0.2pt](C) {\textcolor{white}{#1}};
\end{tikzpicture}
}

\usepackage{xstring}
\newcommand{\PP}[1]{
\vspace{2px}
\noindent{\bf \IfEndWith{#1}{.}{#1}{#1.}}
}

\newcommand{\V}{\checkmark}

==> cvpr/hdr.tex <==
%\icmltitle{Specialization}

% when 'make draft'
\ifdefined\DRAFT
 \pagestyle{fancyplain}
 \lhead{Rev.~\therev}
 \rhead{\thedate}
 \cfoot{\thepage\ of \pageref{LastPage}}
\fi

% blind
% \author{Paper \#123}

\author{
Authors
}



==> cvpr/macros.tex <==
\newcommand{\tts}[1]{\texttt{\small #1}}

\definecolor{Orange}{rgb}{1,0.5,0}
\definecolor{Gray}{rgb}{0.5,0.5,0.5}
\definecolor{LtGray}{rgb}{0.66,0.66,0.66}
\definecolor{Red}{rgb}{0.8,0,0}
\definecolor{Blue}{rgb}{0,0,0.9}
\definecolor{Green}{rgb}{0,0.33,0}

%\newcommand{\w}[1]{{#1}}

\newcommand{\brok}[1]{\sout{#1}}
\newcommand{\cbrok}[1]{\textcolor{Gray}{\brok{#1}}}
\newcommand{\less}[1]{\ensuremath{\check{#1}}}
\newcommand{\cless}[1]{\textcolor{Gray}{\less{#1}}}
\newcommand{\ok}[1]{#1}
\newcommand{\cok}[1]{\ok{#1}}

\renewcommand{\b}[1]{\cbrok{#1}}
\renewcommand{\l}[1]{\cless{#1}}
\renewcommand{\o}[1]{\cok{#1}}

\newcommand{\vhead}[1]{\begin{sideways}#1\end{sideways}}
%\newcommand{\nl}[]{\\&&&}
\newcommand{\none}{-}
\newcommand{\broken}{\ensuremath{\otimes}}
\newcommand{\lessfunc}{\ensuremath{\circleddash}}
\newcommand{\phone}{Phone \#}
\newcommand{\histbookmarks}{Bookmarks}
\newcommand{\sms}{SMS}
\newcommand{\imei}{Device ID}
\newcommand{\location}{Location}
\newcommand{\contacts}{Contacts}
\newcommand{\calendar}{Calendar}
\newcommand{\verify}[1]{\textcolor{Red}{#1}}

\newcommand{\sur}[0]{S}
\newcommand{\cov}[0]{C}
\newcommand{\ove}[0]{O}

\newcommand{\ooo}[0]{\o{\sur}\o{\cov}\o{\ove}}
\newcommand{\ool}[0]{\o{\sur}\o{\cov}\l{\ove}}
\newcommand{\oob}[0]{\o{\sur}\o{\cov}\b{\ove}}
\newcommand{\olo}[0]{\o{\sur}\l{\cov}\o{\ove}}
\newcommand{\oll}[0]{\o{\sur}\l{\cov}\l{\ove}}
\newcommand{\olb}[0]{\o{\sur}\l{\cov}\b{\ove}}
\newcommand{\obo}[0]{\o{\sur}\b{\cov}\o{\ove}}
\newcommand{\obl}[0]{\o{\sur}\b{\cov}\l{\ove}}
\newcommand{\obb}[0]{\o{\sur}\b{\cov}\b{\ove}}

\newcommand{\loo}[0]{\l{\sur}\o{\cov}\o{\ove}}
\newcommand{\lol}[0]{\l{\sur}\o{\cov}\l{\ove}}
\newcommand{\lob}[0]{\l{\sur}\o{\cov}\b{\ove}}
\newcommand{\llo}[0]{\l{\sur}\l{\cov}\o{\ove}}
%\newcommand{\lll}[0]{\l{\sur}\l{\cov}\l{\ove}} % orange?
\newcommand{\llll}[0]{\l{\sur}\l{\cov}\l{\ove}} % orange?
\newcommand{\llb}[0]{\l{\sur}\l{\cov}\b{\ove}} % orange?
\newcommand{\lbo}[0]{\l{\sur}\b{\cov}\o{\ove}}
\newcommand{\lbl}[0]{\l{\sur}\b{\cov}\l{\ove}} % orange?
\newcommand{\lbb}[0]{\l{\sur}\b{\cov}\b{\ove}} % orange?

\newcommand{\boo}[0]{\b{\sur}\o{\cov}\o{\ove}}
\newcommand{\bol}[0]{\b{\sur}\o{\cov}\l{\ove}}
\newcommand{\bob}[0]{\b{\sur}\o{\cov}\b{\ove}}
\newcommand{\blo}[0]{\b{\sur}\l{\cov}\o{\ove}}
\newcommand{\bll}[0]{\b{\sur}\l{\cov}\l{\ove}}  % orange?
\newcommand{\blb}[0]{\b{\sur}\l{\cov}\b{\ove}}  % orange?
\newcommand{\bbo}[0]{\b{\sur}\b{\cov}\o{\ove}}
\newcommand{\bbl}[0]{\b{\sur}\b{\cov}\l{\ove}}  % orange?
\newcommand{\bbb}[0]{\textcolor{red}{\brok{\sur}\brok{\cov}\brok{\ove}}}

\newcommand{\sys}{\mbox{MetaSync}\xspace}
\newcommand{\syss}{\mbox{metasync}\xspace}
\newcommand{\sysr}{\mbox{\tt .metasync}\xspace}
\newcommand{\tomcomment}[1]{\textcolor{Blue}{[tom: #1]}}
\newcommand{\akcomment}[1]{\textcolor{Blue}{[ak: #1]}}
\newcommand{\TK}[1]{\textcolor{Blue}{[TK: #1]}}
\newcommand{\XXX}{\textcolor{Red}{XXX }}

\newcommand{\vladd}[1]{\textcolor{cyan}{#1}}
\newcommand{\vlremove}[1]{\textcolor{Gray}{\sout{#1}}}
\newcommand{\vlreplace}[2]{\textcolor{Gray}{\sout{#1}}\textcolor{cyan}{#2}}
\newcommand{\vlcomment}[1]{\textcolor{Orange}{[vl: #1]}}

\newcommand{\shadd}[1]{\textcolor{magenta}{#1}}
\newcommand{\shremove}[1]{\textcolor{Gray}{\sout{#1}}}
\newcommand{\shreplace}[2]{\textcolor{Gray}{\sout{#1}}\textcolor{magenta}{#2}}
\newcommand{\shcomment}[1]{\textcolor{Orange}{[seungyeop: #1]}}
\newcommand{\haichen}[1]{\textcolor{Blue}{[haichen: #1]}}
\newcommand{\arvind}[1]{\textcolor{red}{[arvind: #1]}}

\newcommand{\osdi}[2]{\textcolor{red}{[OSDI R#1: #2]}}

\newcommand{\remove}[1]{}
% To show changes in the document, comment out the \renewcommand definitions below
%\renewcommand{\vladd}[1]{#1}
%\renewcommand{\vlremove}[1]{}
%\renewcommand{\vlreplace}[2]{#2}
%\renewcommand{\vlcomment}[1]{}

%\renewcommand{\shadd}[1]{#1}
%\renewcommand{\shremove}[1]{}
%\renewcommand{\shreplace}[2]{#2}
%\renewcommand{\shcomment}[1]{}
%\renewcommand{\TK}[1]{}
%\renewcommand{\osdi}[2]{}

%\renewcommand{\aladd}[1]{#1}
%\renewcommand{\alremove}[1]{}
%\renewcommand{\alreplace}[2]{#2}
%\renewcommand{\alcomment}[1]{}

% autoref
\def\Snospace~{Section~{}}
\renewcommand*\sectionautorefname{\Snospace}
\def\sectionautorefname{\Snospace}
\def\subsectionautorefname{\Snospace}
\def\subsubsectionautorefname{\Snospace}
\def\chapterautorefname{\Snospace}
\def\algorithmautorefname{Algorithm}

% various lists
\newcommand{\squishlist}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{0pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishnone}{
   \begin{list}{}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{0pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{0em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishlistcirc}{
   \begin{list}{$\circ$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{0pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishlisttwo}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}    \setlength{\parsep}{0pt}
      \setlength{\topsep}{0pt}     \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{2em} \setlength{\labelwidth}{1.5em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishend}{
    \end{list} \vspace{5pt} }
%\ifpdf
%\setlength{\pdfpagewidth}{8.5in}
%\setlength{\pdfpageheight}{11in}
%\else
%\fi

\newcommand{\includepdf}[1]{
  \includegraphics[width=\columnwidth]{#1}
}
\newcommand{\includeplot}[1]{
  \resizebox{\columnwidth}{!}{\input{#1}}
}

% use \cc instead of \texttt
\newcommand{\cc}[1]{\mbox{\smaller[0.5]\texttt{#1}}}
\newcommand{\cC}[1]{\mbox{\smaller[0.6]\texttt{#1}}}



% common rules
\newcommand{\figrule}{\hrule width \hsize height .33pt \vspace{5px}}
\newcommand{\coderule}{\vspace{-0.4em}\figrule}



==> cvpr/pkgs.tex <==
\input{warning}

\usepackage[hyphens]{url}
\usepackage[breaklinks,colorlinks]{hyperref}
%\usepackage[usenames,dvipsnames]{xcolor}
\hypersetup{citecolor=blue,linkcolor=blue}
\usepackage{amsmath,amsopn,amssymb}
\usepackage{subfigure}
\usepackage{endnotes,microtype,xspace,graphicx,fancyvrb,multirow}
\usepackage{booktabs}
\usepackage{array,underscore,relsize}
\usepackage[T1]{fontenc}
\usepackage{times}
\usepackage{fancyhdr,lastpage}
\usepackage{enumitem}
\usepackage[labelfont=bf,font=small,skip=5pt]{caption}
\pagestyle{fancy}
\fancyhf{}
\renewcommand{\headrulewidth}{0pt}
\cfoot{\thepage}


==> cvpr/problem.tex <==
\section{The sequential model specialization problem}
\label{s:problem}
We approach model specialization as a pair of loosely coupled problems. One is a sequential decision making problem to detect skews and select optimal models, and the other is a cost-sensitive classification problem to produce these models.

Let $x_1,x_2,\ldots,x_i,\ldots \in X = \mathbb{R}^{n}$ be a stream of values to be classified. Let $y_1,y_2,\ldots,y_i,\ldots \in Y= [1,\ldots,k]$ be the corresponding classification results. Let $\pi: \mathbb{I^+} \to \mathbb{I^+}$ be a partition over the values. Associate the distribution $T_j$ with partition $j$, so that each pair $(x_i,y_i)$ is sampled from $T_{\pi(i)}$. Intuitively, $\pi$ partitions, or segments, $\ldots, x_i, \ldots$ into a sequence of ``epochs'', where elements from each epoch $j$ are drawn independently from the corresponding stationary distribution $T_j$. Thus, for the overall series, samples are drawn from an abruptly-changing, piece-wise stationary distribution. At test time, we assume neither results $y_i$ nor partitions $\pi$ are known.

Let $h^*:X \to Y$ be a classifier, designated the ``oracle'' classifier, trained on distribution $T^*$. Intuitively $T^*$ is a mixture of all distributions comprising the oracle's input stream: $T^* = \sum_{j} T_j$. Let $R(h^*)$ be the resources (e.g., execution cycles), assumed invariant across $X$, needed to execute $h^*$ on any $x \in X$. Executing $h^*$ incurs a cost of $R(h^*)$ with probability 1. At test time, on each input $x_i$, we can always consult $h^*$ at cost $R(h^*)$ to get a label $y_i$ with accuracy $a^*$ on average.

Alternately, we are free to consult one of many available ``specialized'' classifiers $h_k$ instead. Intuitively, a non-stationary distribution $T_j$ would likely have an associated specialized classifier that, on average, requires substantially fewer resources than the oracle on samples from that distribution. For simplicity, we assume for now that $h_k$ agrees with $h^*$ on all inputs $x$. Further, we require that for a given epoch $j$, the overhead $R(h_k)$ of executing $h_k$ on input $x_i$ can take one of two fixed values, $(R_-,R_+)$ with probabilities $(p_{kj}, 1-p_{kj})$. Intuitively, we expect that  specialized models will have some inputs they ``do well'' on, and others they do poorly on, corresponding to lower versus higher resource costs. Finally, we require that $R_- \leq R(h^*) \leq R_+$ (specialized models whose best-case resource use exceed that of the oracle are useless), and that each specialized model $h_k$ must have some epoch $j$  where this holds  with high probability $p_{kj}$, ideally with $R_- \ll R(h^*)$. 

The overall problem is to select a model (whether specialized or oracle) to process each input $x_i$ such that the aggregate resource use across all inputs is minimized. Ignoring details of how specialized models are obtained (and the cost of doing so), this problem can be framed as a piece-wise stationary multi-armed bandit problem  \cite{garivier2008upper}. Each classifier $h_k$ (including the oracle, which can be regarded as $h_0$) is an arm of the bandit. The cost-distribution of arm $k$ during the $j$-th stationary epoch is  $(R_-,R_+)$ with a priori unknown probabilities $(p_{kj}, 1-p_{kj})$. Let $h^*_j$ be the specialized model with lowest resource use for epoch $j$. If $h_i$ is the classifier selected by our algorithm to process $x_i$, we wish to minimize the regret  $\sum_i R(h_i)-R(h^*_{\pi(i)})$.

For regret to be low in absolute terms, the bandit scheme above requires that for any input distributions $T_j$ it may encounter, it has access to specialized classifier $h_k$ such that $h_k$ has low overhead $R_-$ with relatively high probability $p_{kj}$. Note, for instance that if all $p_{kj}$ were zero, regret would be at least as much as using the oracle on every input, so that the specialized classifier would consume at least as many resources as the oracle. Further, the above setup requires that the specialized models are at least as accurate as the oracle over {\em any} input, and vary only in the resources required to process the input. Although in our solution below we are not able to meet this ideal, we are able to provide $h_k$'s that match the oracle for specific epochs. This relaxation still allows useful solutions to the problem. 

If the $T_j$ were known offline, one could imagine training some form of cost-sensitive classifier that is especially cheap on a skewed distribution $T_j$ with high probability. Note however, that the number of distributions to specialize over (i.e., the number of distributions $T_j$) is very large when the number of classes is large, even assuming techniques like quantization of distributions. Thus, in the case we address below, the $T_j$ are inferred online by the bandit, and we need to {\em train} corresponding specialized classifiers $h_k$ online. This brings up the challenging requirement that training overhead be minimized (since the bandit cannot provide access to the arm before it is done training) while ensuring that the resulting model is accurate as well. Further, if $R_T$ is the training cost, the bandit scheme needs to assess a one-time cost of $R_T$ to access the model for the first time. 

Below, we provide a framework that heuristically combines an exploration/exploitation scheme with a novel cascaded classifier to find and exploit opportunities for sequential model specialization.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../nips_p"
%%% End: 


==> cvpr/rev.tex <==
\gdef\therev{39a40c2}
\gdef\thedate{2016-05-11 16:05:29 -0700}


==> cvpr/specialize.tex <==
\subsection{Specializer}
\label{s:specializer}
%1. How to specialize a model to a subset of labels? (training)
%We first trained the lower layers of the small model over entire dataset. Then retarget the last layer over the skewed data set.
%2. Show the training overhead. How long does it take for specialization? It is proportional to the number of in-context classes and number of training samples per class.

In this section, we describe how the system prepares a special model through the specializer. 
Specialization takes two steps: (1) training the lower layers of a compact model over the entire dataset, (2) re-targeting the last layers over the skewed dataset.
Note that the first step is done off-line, and only the second step needs to be done at runtime. 

The specializer maintains pretrained bottom layers of compact models. 
Once the context monitor detects a skew, it provides the specializer with in-context labels and skewness to use.
Then, the specializer trains the last layers based on the information. 
It composes layers with a fully connected layer and a softmax layer to provide recognition output. 
Output classes include all in-context labels and \textit{other} label which indicates that the input does not belong to in-context labels.
A training set is prepared as a mix of images from the in-context labels and images randomly picked from out-context, and the proportion follows the given skewness.  To prepare, each image is forwarded through the bottom layers and the forwarded result is used in retargeting the last layers.  The forwarding step takes longer than retargeting in general, but forwarded result can be prepared in advance.  Finally, because the number of parameters to train is not huge for the last layer, retargeting does not need the whole training set for the in-context labels, but it needs to use a subset of it.  

%\shcomment{I'll add training cost (latency), and some accuracies}


==> cvpr/support.tex <==

\section*{Supplementary Material}
\label{app:support}

We use a simple model to analyze how to choose the minimum support number $c$
for different window sizes $w$ in order to limit the number of specialized models to
be evaluated in \autoref{alg:opt-alg} during exploration. Suppose $N$ is the
number of total classes classified by the oracle $h^*$ and that the accuracy of $h^*$
is $a^*$. If the classification result by the oracle is wrong, the probability that
the oracle classifies the input to each of the other classes is assumed to be equivalent. Assume the
input sequences are drawn independently from a skewed distribution $T$ which has
$n$ dominant classes with skew $p$. Denote the dominant set as $\mathcal{S}$
and non-dominant set as $\mathcal{O}$. Among dominant or non-dominant set,
the probability of each class is assumed to be the same. Based on
these definitions, we can compute the probability of any single class being
classified. Similar to Equation 1 in the paper, consider one dominant class
$\ell$, the probability that it will be classified by the oracle is:
\begin{align}
  p(\ell \in \mathcal{S}) &= \frac{1}{n} \cdot \hat{p} = \frac{1}{n} \left(p\cdot a^* + p(1-a^*)\frac{n-1}{N-1}
  + (1-p)(1-a^*)\frac{n}{N-1}\right)
  \label{eq:in-context-prob}
\end{align}
%% The first term in \autoref{eq:in-context-prob} indicates that the input belongs
%% to $\mathcal{I}$ and is recognized correctly. The second term is when the input
%% belongs to $\mathcal{I}$ and the recognition result is wrong but still among
%% $\mathcal{I}$. The third term shows that the input belongs to out-context
%% classes $\mathcal{O}$ and is recognized as an in-context class. The sum of these
%% three terms gives the probability of all in-context classes being predicted. To
%% compute the probability of a single in-context class, we need to divide it by
%% $k$.
And we can compute the probability of a non-dominant class $\ell'$ being
classified by:
\begin{align}
  p(\ell' \in \mathcal{O}) &= \frac{1}{N-n} \left((1-p)a^* + (1-p)(1-a^*)\frac{N-n-1}{N-1}
  + p(1-a^*)\frac{N-n}{N-1}\right)
  \label{eq:out-context-prob}
\end{align}
From \autoref{eq:in-context-prob} and \ref{eq:out-context-prob}, we can then
calculate the probability of a dominant class or a non-dominant class that is
classified at least $c$ times in the window $w$ by treating it as a binomial
distribution. Intuitively, we hope the probability of a dominant class that is
classified at least $c$ times ($p_{in}$) be as high as possible, while the
probability of any non-dominant class ($p_{out}$) be as low as possible. We
considered different combinations of $N, a^*, n, p$ under different $w$ and $c$
settings, and computed $p_{in}$ and $p_{out}$. \autoref{tab:window-support}
shows how $p_{in}$ and $p_{out}$ changes under different settings. From the
table, we can tell that with an increase in the number of dominant classes and a
decrease in skew, we need to increase the size of window to have a higher
probability that the dominant classes can be detected in the window. However,
when the window size is larger, we also need to increase the minimum support
number $c$ (Row 6 and 7) to limit the probability that a non-dominant class
appears $c$ times. In addition, when there is no skew in the distribution (Row
8), the minimum support number $c$ is also effective at filtering out most of
the non-dominant classes. In practice, we set $c=2$ for $w < 90$ and $c=3$ for
$w\geq 90$.

\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{5pt}
\begin{tabular}{ccccccccc}
  \toprule
  index & $N$ & $a$ & $n$ & $p$ & $w$ & $c$ & $p_{in}$ & $p_{out}$\\\midrule
  1 & 1000 & 0.68 & 5 & 0.9 & 30 & 2 & 0.896 & 6.52E-5\\
  2 & 1000 & 0.68 & 10 & 0.9 & 30 & 2 & 0.558 & 6.53E-5\\
  3 & 1000 & 0.68 & 10 & 0.9 & 60 & 2 & 0.891 & 2.64E-4\\
  4 & 1000 & 0.68 & 10 & 0.7 & 60 & 2 & 0.789 & 4.80E-4\\
  5 & 1000 & 0.68 & 10 & 0.7 & 90 & 2 & 0.933 & 1.08E-3\\
  6 & 205 & 0.58 & 10 & 0.9 & 90 & 2 & 0.959 & 0.019\\
  7 & 205 & 0.58 & 10 & 0.9 & 90 & 3 & 0.872 & 1.31E-3\\
  8 & 205 & 0.58 & 0 & N/A & 90 & 3 & N/A & 9.29E-3\\\bottomrule
\end{tabular}
\vspace{5pt}
\caption{Probability $p_{in}$ and $p_{out}$ under various $N,a,n,p$ and $w,c$.
  In row 8, $k=0$ and $p=$ N/A indicates that the distribution has no
  skew and is uniform across all $N$ classes.}
\label{tab:window-support}
\end{table}


==> cvpr/system.tex <==
\section{System Design}
\label{s:system}

\begin{figure}[t]
\centering
\includegraphics[width=.9\textwidth]{figures/system_overview.pdf}
\caption{System overview}
\label{fig:sys-overview}
\end{figure}

To exploit the temporal class skews in streaming videos during run time,
we designed a generic system shown in \autoref{fig:sys-overview}. 
In this section, we first describe the overall work flow of our system and 
then explain the details of the system modules in the following sections.
In \autoref{fig:sys-overview}, the white boxes and solid arrows show the data 
flow of the image recognition process, whereas the gray boxes and dotted arrows 
show the control flow of the runtime system.

Given a frame, the system looks up whether there exists a compact classifier 
to use. A compact classifier is trained to recognize a subset of classes which 
have appeared frequently in the recent history; we refer to this subset of labels as 
\textit{in-context labels}. Compact classifiers are designed to be much smaller 
than the complete classifier in both memory usage and computational needs, hence they 
take less time and resources to run. If there is a compact classifier available, 
the system will first run the compact classifier. If the output belongs to one of the 
in-context classes, the system directly uses it as the recognition result; otherwise, 
it will then run the complete classifier in a cascaded manner. If there is no 
appropriate compact classifier available at run time, the system will simply run the complete 
classifier and use its output as the classification result.

The classification output is also used as a feedback signal in the
control loop. The context monitor keeps track of the output history
and provides a distribution of the recognized classes when the
decision engine queries it with a history window size.  The decision
engine adaptively selects a window size, and decides when to train a
new compact classifier and when to stop using the current compact
classifier based on the distribution obtained from the context
monitor. Given the class distribution, the decision engine estimates
the current short-term skew and the accuracy that a compact classifier
can achieve under the skew. If the estimated accuracy of a compact
classifier is higher than the accuracy of the complete one, the
decision engine tells the specializer to train a compact
classifier. During the time it takes to perform training, the system
still uses the complete classifier to process incoming requests. Once
specialization is complete, the system uses the compact classifier as
the first element of a chained classifier.  While the compact
classifier is being used, the decision engine keeps monitoring the
skew of in-context classes and the estimated accuracy. Once it detects
changes in the skew and if the estimated accuracy of the compact
classifier falls below the accuracy of the complete classifier, the
decision engine will stop using the compact classifier and the system
switches back to using just the complete classifier.

To build a system that can adaptively generate a compact classifier based
on temporal short-term skews, we need to address the following three challenges:
\begin{itemize}[label=$\bullet$]
\item Can we generate classifiers for in-context classes that are much smaller and more accurate than the complete classifier?
\item Can we train a compact classifier fast enough to be used in
  response to changes in temporal class skews?
\item Can we detect short-term class skews during run time?
\end{itemize}
In \autoref{s:cnn}, we show that we can generate much more compact
classifiers that achieve higher accuracy in recognizing in-context
classes. \autoref{s:specializer} explains the performance
optimization that we use in the specializer. The results show that
training can be fast enough to generate a compact classifier during
run time.  \autoref{s:skew_detection} describes the operation of the
context monitor and the decision engine, and also outlines the
algorithm to detect the skews.


==> cvpr/table_stats.tex <==
\begin{tabular}{cccccc}
  \toprule
  Videos & special rate & cascade rate & special times & dominant set size & window size \\
  \midrule
  Friends & 86.5\% & 8.8\% & 46 & 2.3 & 47.0 \\
  Good Will Hunting & 95.6\% & 5.6\% & 6 & 2.0 & 30.0 \\
  Ellen Show & 99.0\% & 5.3\% & 3 & 1.3 & 30.0 \\
  The Departed & 92.2\% & 7.2\% & 8 & 2.4 & 37.5 \\
  Ocean's Eleven / Twelve & 82.8\% & 17.0\% & 15 & 1.8 & 44.0 \\
  \bottomrule
\end{tabular}


==> cvpr/warning.tex <==
\usepackage{silence}
\WarningFilter*{caption}{Unsupported document class}

==> hdr.tex <==
%\icmltitle{Specialization}

% when 'make draft'
\ifdefined\DRAFT
 \pagestyle{fancyplain}
 \lhead{Rev.~\therev}
 \rhead{\thedate}
 \cfoot{\thepage\ of \pageref{LastPage}}
\fi

% blind
% \author{Paper \#123}

\author{
Authors
}


